Link homology and Frobenius extensions II

The first two sections of the paper provide a convenient scheme and additional diagrammatics for working with Frobenius extensions responsible for key flavors of equivariant SL(2) link homology theories. The goal is to clarify some basic structures in the theory and propose a setup to work over sufficiently non-degenerate base rings. The third section works out two related SL(2) evaluations for seamed surfaces.

==> cf_cube-non-hom.tex <==
\begin{scope}
  \begin{scope}
    \coordinate (a) at ( 0.500, 0.500);
    \coordinate (b) at (-0.500, 0.500);
    \coordinate (c) at (-0.500,-0.500);
    \coordinate (d) at ( 0.500,-0.500);
    \coordinate (A) at ( 1, 1);
    \coordinate (B) at (-1, 1);
    \coordinate (C) at (-1,-1);
    \coordinate (D) at ( 1,-1);
  \end{scope}
  
  \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm,
    segment length=0.5mm}, thick]
    \draw[decorate] (c) -- (d);
    \draw[decorate] (a) -- (b);
    \draw[decorate] (C) -- (D);
    \draw[decorate] (A) -- (B);
  \end{scope}
  
  \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
    \draw[decorate] (a) -- (d);
    \draw[decorate] (c) -- (b);
    \draw[decorate] (A) -- (D);
    \draw[decorate] (C) -- (B);
  \end{scope}
  
  \begin{scope}[blue, thick]
    \draw[double] (a) -- (A);
    \draw[double] (b) -- (B);
    \draw[double] (c) -- (C);
    \draw[double] (d) -- (D);
  \end{scope}
\end{scope}
\begin{scope}[xshift=5cm]
  \begin{scope}
    \coordinate (a) at ( 0.500, 0.500);
    \coordinate (b) at (-0.500, 0.500);
    \coordinate (c) at (-0.500,-0.500);
    \coordinate (d) at ( 0.500,-0.500);
    \coordinate (A) at ( 1, 1);
    \coordinate (B) at (-1, 1);
    \coordinate (C) at (-1,-1);
    \coordinate (D) at ( 1,-1);
  \end{scope}
  
  \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm,
    segment length=0.5mm}, thick]
    \draw[decorate] (c) -- (b);
    \draw[decorate] (a) -- (d);
    \draw[decorate] (C) -- (D);
    \draw[decorate] (A) -- (B);
  \end{scope}
  
  \begin{scope}[red, decoration={zigzag, segment length=1.5mm,
    amplitude=0.3mm}, thick, decorate]
    \draw[decorate] (a) -- (b);
    \draw[decorate] (c) -- (d);
    \draw[decorate] (A) -- (D);
    \draw[decorate] (C) -- (B);
  \end{scope}
  
  \begin{scope}[blue, thick]
    \draw[double] (a) -- (A);
    \draw[double] (b) -- (B);
    \draw[double] (c) -- (C);
    \draw[double] (d) -- (D);
  \end{scope}
\end{scope}    

==> cf_digon.tex <==
\begin{scope}
    \begin{scope}
        \draw (-1,0) -- (-0.5, 0) .. controls +(0.3, 0.3) and + (-0.3, 0.3) .. (0.5,0) -- (1,0);
        \draw (-0.5, 0) .. controls +( 0.3, -0.3) and + (-0.3, -0.3) .. (0.5,0);
        \node[below] at (0, -0.3) {$\Gamma$};
    \end{scope}
  %  \node at (2.5, 0) {$\leftrightsquigarrow$}; 
    \begin{scope}[xshift = 5cm]
        \draw (-1,0) -- (1,0);
        \node[below] at (0, -0.3) {$\Gamma'$};
    \end{scope}
\end{scope}

==> cf_square.tex <==
\begin{scope}[scale =0.8]
    \begin{scope}
        \draw (0.5,-0.5) -- (0.5,0.5) -- (-0.5, 0.5) -- (-0.5, -0.5) -- (0.5, -0.5);
        \draw (0.5, 0.5) -- (1,1);
        \draw (-0.5, 0.5) -- (-1,1);
        \draw (0.5, -0.5) -- (1,-1);
        \draw (-0.5, -0.5) -- (-1,-1);
        \node at (0, -1.3) {$\Gamma$};
    \end{scope}
    %\node at (2.5, 0) {$\leftrightsquigarrow$}; 
    \begin{scope}[xshift = 6cm]
        \draw (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
        \draw (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
        \node at (0, -1.3) {$\Gamma_v$};
    \end{scope}
    \begin{scope}[xshift = 12cm]
        \draw (1, -1) .. controls +(-0.5, 0.5) and +(0.5, 0.5) .. (-1,-1);
        \draw (1,  1) .. controls +(-0.5, -0.5) and +(0.5, -0.5) .. (-1,1);
        \node at (0, -1.3) {$\Gamma_h$};
    \end{scope}
\end{scope}

==> cf_square2.tex <==
\begin{scope}[scale =0.8]
  \begin{scope}
    \node[black] at (0, -1.3) {$c$}; 
        \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick]
            \draw[decorate] (0.5,-0.5) -- (0.5,0.5);
            \draw[decorate] (-0.5, -0.5) -- (-1,-1);
            \draw[decorate] (-0.5, 0.5) -- (-1,1);
        \end{scope}
        \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
            \draw[decorate] (-0.5, 0.5) -- (-0.5, -0.5);
            \draw[decorate] (0.5, 0.5) -- (1,1);
            \draw[decorate] (0.5, -0.5) -- (1,-1);
        \end{scope}
        \begin{scope}[blue, thick]
            \draw[double] (0.5, 0.5) -- (-0.5, 0.5);
            \draw[double] (-0.5, -0.5) -- (0.5, -0.5);
        \end{scope}
    \end{scope} 
  \node at (-2.5, 0) {$\leftsquigarrow$};
  \node at (+7.5, 0) {$\rightsquigarrow$};    
  \begin{scope}[xshift = 5cm, rotate = 90]
        \node[black] at ( -1.3, 0) {$c$}; 
        \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick]
            \draw[decorate] (0.5,-0.5) -- (0.5,0.5);
            \draw[decorate] (-0.5, -0.5) -- (-1,-1);
            \draw[decorate] (-0.5, 0.5) -- (-1,1);
        \end{scope}
        \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
            \draw[decorate] (-0.5, 0.5) -- (-0.5, -0.5);
            \draw[decorate] (0.5, 0.5) -- (1,1);
            \draw[decorate] (0.5, -0.5) -- (1,-1);
        \end{scope}
        \begin{scope}[blue, thick]
            \draw[double] (0.5, 0.5) -- (-0.5, 0.5);
            \draw[double] (-0.5, -0.5) -- (0.5, -0.5);
        \end{scope}
    \end{scope} 
  \begin{scope}[xshift =10cm, rotate=90,  red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
    \node[black] at ( -1.3, 0) {$c_h$}; 
    \draw[red, decoration={zigzag, segment length=1.5mm,
    amplitude=0.3mm}, thick, decorate] (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
    \draw[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick,decorate] (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
  \end{scope}
  \begin{scope}[xshift = -5cm,  red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
    \node[black] at ( 0,-1.3) {$c_v$}; 
    \draw[red, decoration={zigzag, segment length=1.5mm,
    amplitude=0.3mm}, thick, decorate] (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
    \draw[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick,decorate] (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
  \end{scope}
\end{scope}

==> cf_square3.tex <==
\begin{scope}[scale =0.8]
  \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
    \draw[decorate] (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
    \draw[decorate] (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
    \node[black] at (0, -1.3) {$c_v$}; 
  \end{scope}
  \node at (-2.5, 0) {$\leftsquigarrow$};
  \node at (+2.5, 0) {$\rightsquigarrow$};
  \begin{scope}[xshift=-5cm]
    \node[black] at (0, -1.3) {$c_1$}; 
    \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick]
      \draw[decorate] (0.5,-0.5) -- (0.5,0.5);
      \draw[decorate] (-0.5, 0.5) -- (-0.5, -0.5);
    \end{scope}
    \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
      \draw[decorate] (-0.5, -0.5) -- (-1,-1);
      \draw[decorate] (-0.5, 0.5) -- (-1,1);
      \draw[decorate] (0.5, 0.5) -- (1,1);
      \draw[decorate] (0.5, -0.5) -- (1,-1);
    \end{scope}
    \begin{scope}[blue, thick]
      \draw[double] (0.5, 0.5) -- (-0.5, 0.5);
      \draw[double] (-0.5, -0.5) -- (0.5, -0.5);
    \end{scope}
  \end{scope} 
  \begin{scope}[xshift = 5cm, rotate = 90]
        \node[black] at ( -1.3, 0) {$c_2$}; 
    \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick]
      \draw[decorate] (0.5,-0.5) -- (0.5,0.5);
      \draw[decorate] (-0.5, 0.5) -- (-0.5, -0.5);
    \end{scope}
    \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
      \draw[decorate] (-0.5, -0.5) -- (-1,-1);
      \draw[decorate] (-0.5, 0.5) -- (-1,1);
      \draw[decorate] (0.5, 0.5) -- (1,1);
      \draw[decorate] (0.5, -0.5) -- (1,-1);
    \end{scope}
    \begin{scope}[blue, thick]
      \draw[double] (0.5, 0.5) -- (-0.5, 0.5);
      \draw[double] (-0.5, -0.5) -- (0.5, -0.5);
    \end{scope}
  \end{scope}
  \begin{scope}[xshift=10cm]
    \draw[red, decoration={zigzag, segment length=1.5mm,
    amplitude=0.3mm}, thick, decorate] (-1, 0.7) -- +(0.5, 0) node[right, black]
    {$1$};
        \draw[blue, thick, double] (-1, 0) -- +(0.5, 0) node[right, black] {$2$};  
    \draw[green!50!black,decoration={coil,amplitude=0.3mm, segment
    length=0.5mm}, thick, decorate] (-1, -0.7) -- +(0.5, 0) node[right, black] {$3$};  
  \end{scope}
\end{scope} 
  
  

==> cf_square4.tex <==
\begin{scope}[scale =0.8]
  % \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
  %   \draw[decorate] (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
  %   \draw[decorate] (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
  %   \node[black] at (0, -1.3) {$c_v$}; 
  % \end{scope}
  % \node at (-2.5, 0) {$\leftsquigarrow$};
  % \node at (+2.5, 0) {$\rightsquigarrow$};
  \begin{scope}[xshift=-5cm]
    \node[black] at (0, -1.3) {$\Gamma_{12}(c_1)$}; 
    \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm,
      segment length=0.5mm}, thick, opacity=0.2]
      \draw[decorate] (0.5,-0.5) -- (0.5,0.5);
      \draw[decorate] (-0.5, 0.5) -- (-0.5, -0.5);
    \end{scope}
    \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
      \draw[decorate] (-0.5, -0.5) -- (-1,-1);
      \draw[decorate] (-0.5, 0.5) -- (-1,1);
      \draw[decorate] (0.5, 0.5) -- (1,1);
      \draw[decorate] (0.5, -0.5) -- (1,-1);
    \end{scope}
    \begin{scope}[blue, thick]
      \draw[double, densely dashed] (-1,1) arc (90:270: 0.8cm and
      1cm);
      \draw[double, densely dashed] (1,1) arc (90:-90: 0.8cm and 1cm);
      \draw[double] (0.5, 0.5) -- (-0.5, 0.5);
      \draw[double] (-0.5, -0.5) -- (0.5, -0.5);
    \end{scope}
  \end{scope} 
  \begin{scope}[xshift = 5cm]
        \node[black] at (0,-1.3) {$\Gamma_{12}(c_2)$}; 
    \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm,
      segment length=0.5mm}, thick, opacity=0.2]
      \draw[decorate] (0.5, 0.5) -- (-0.5, 0.5);
      \draw[decorate] (-0.5, -0.5) -- (0.5, -0.5);
    \end{scope}
    \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
      \draw[decorate] (-0.5, -0.5) -- (-1,-1);
      \draw[decorate] (-0.5, 0.5) -- (-1,1);
      \draw[decorate] (0.5, 0.5) -- (1,1);
      \draw[decorate] (0.5, -0.5) -- (1,-1);
    \end{scope}
    \begin{scope}[blue, thick]
      \draw[double, densely dashed] (-1,1) arc (90:270: 0.8cm and
      1cm);
      \draw[double, densely dashed] (1,1) arc (90:-90: 0.8cm and 1cm);
      \draw[double] (0.5,-0.5) -- (0.5,0.5);
      \draw[double] (-0.5, 0.5) -- (-0.5, -0.5);
    \end{scope}
  \end{scope}
  % \begin{scope}[xshift=10cm]
  %   \draw[red, decoration={zigzag, segment length=1.5mm,
  %   amplitude=0.3mm}, thick, decorate] (-1, 0.7) -- +(0.5, 0) node[right, black]
  %   {$1$};
  %       \draw[blue, thick, double] (-1, 0) -- +(0.5, 0) node[right, black] {$2$};  
  %   \draw[green!50!black,decoration={coil,amplitude=0.3mm, segment
  %   length=0.5mm}, thick, decorate] (-1, -0.7) -- +(0.5, 0) node[right, black] {$3$};  
  % \end{scope}
\end{scope} 
  
  

==> cf_square5.tex <==
\begin{scope}[scale =0.8]
  \begin{scope}[xshift =-5cm, red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
    \draw[decorate] (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
    \draw[decorate] (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
    \node[black] at (0, -1.3) {$c_v$}; 
  \end{scope}
  \node at (-2.5, 0) {$\leftsquigarrow$};
  \node at (+2.5, 0) {$\rightsquigarrow$};
  \begin{scope}[xshift=0cm]
    \node[black] at (0, -1.3) {$c$}; 
    \begin{scope}[green!50!black,decoration={coil,amplitude=0.3mm, segment length=0.5mm}, thick]
      \draw[decorate] (0.5,-0.5) -- (0.5,0.5);
      \draw[decorate] (-0.5, 0.5) -- (-0.5, -0.5);
    \end{scope}
    \begin{scope}[red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]
      \draw[decorate] (-0.5, -0.5) -- (-1,-1);
      \draw[decorate] (-0.5, 0.5) -- (-1,1);
      \draw[decorate] (0.5, 0.5) -- (1,1);
      \draw[decorate] (0.5, -0.5) -- (1,-1);
    \end{scope}
    \begin{scope}[blue, thick]
      \draw[double] (0.5, 0.5) -- (-0.5, 0.5);
      \draw[double] (-0.5, -0.5) -- (0.5, -0.5);
    \end{scope}
  \end{scope} 
  \begin{scope}[xshift = 5cm, rotate = 90,  red, decoration={zigzag, segment length=1.5mm, amplitude=0.3mm}, thick]]
    \node[black] at ( -1.3, 0) {$c_h$}; 
    \draw[decorate] (1, -1) .. controls +(-0.5, 0.5) and +(-0.5, -0.5) .. (1,1);
    \draw[decorate] (-1,  -1) .. controls +(0.5, 0.5) and +(0.5, -0.5) .. (-1,1);
  \end{scope}
\end{scope} 
  
  

==> cf_theta-split.tex <==
\begin{scope}
  \begin{scope}[yshift= 1.5cm]
    \draw (1,0) arc (0:360:1cm and 0.3cm) coordinate[pos=0.2] (a)
    coordinate[pos=0.7] (b);
    \draw[thin] (1,0) arc (0:-180:1cm and 1.2cm) coordinate[pos=0.5] (c);
    \draw (a) .. controls +(0,0) and +(0.2,0) .. (c) .. controls
    +(-0.2, 0) and +(0,0) .. (b) --(a);
  \end{scope}
  \begin{scope}[yshift =-1.5cm]
    \draw (1,0) arc (0:360:1cm and 0.3cm) coordinate[pos=0.2] (a)
    coordinate[pos=0.7] (b);
    \draw (1,0) arc (0:180:1cm and 1.2cm) coordinate[pos=0.5] (c);
    \draw (a) .. controls +(0,0) and +(0.2,0) .. (c) .. controls
    +(-0.2, 0) and +(0,0) .. (b) --(a);
  \end{scope}
\end{scope}

==> cf_triangle.tex <==
\begin{scope}
    \begin{scope}
        \draw (0,0) -- (90:1);
        \draw (0,0) -- (-30:1);
        \draw (0,0) -- (-150:1);
        \node at (0, -1) {$\Gamma$};
    \end{scope}
    %\node at (2.5, 0) {$\leftrightsquigarrow$}; 
    \begin{scope}[xshift = 5cm]
        \draw (90:0.7) -- (90:1);
        \draw (-30:0.7) -- (-30:1);
        \draw (-150:0.7) -- (-150:1);
        \draw (90: 0.7)--(-30: 0.7) -- (-150: 0.7)-- cycle;
        \node at (0, -1) {$\Gamma'$};
    \end{scope}
\end{scope}

==> cf_triangle2.tex <==
\begin{scope}
    \begin{scope}
        \draw (0,0) -- (90:1);
        \draw (0,0) -- (-30:1);
        \draw (0,0) -- (-150:1);
    \end{scope}
    \node at (2.5, 0) {$\rightsquigarrow$}; 
    \begin{scope}[xshift = 5cm]
        \draw (90:0.7) -- (90:1);
        \draw (-30:0.7) -- (-30:1);
        \draw (-150:0.7) -- (-150:1);
        \draw (90: 0.7)--(-30: 0.7) -- (-150: 0.7)-- cycle;
    \end{scope}
\end{scope}

==> fe_twisted-tube-2pt.tex <==
\begin{scope}
\begin{scope}  [decoration={border,segment length=1mm,amplitude=1mm,angle=-90}]
  \begin{scope}[xshift=0cm]
    \draw (1,0) arc (0:360:1cm and 0.3cm)coordinate [pos=0](e)
    coordinate [pos=0.5](f) coordinate[pos=0.65] (bl)
    coordinate[pos=0.85] (al);
    \draw[very thin] (-1,0) arc (180:270:1cm and 1.2cm) coordinate[pos=1] (LB);
  \end{scope}
    \begin{scope}[xshift=2.5cm]
    \draw (1,0) arc (0:360:1cm and 0.3cm)coordinate [pos=1](f)
    coordinate [pos=0.5](f) coordinate[pos=0.65] (br)
    coordinate[pos=0.85] (ar);
    \draw[very thin] (1,0) arc (0:-90:1cm and 1.2cm) coordinate[pos=1]
    (RB);
  \end{scope}
  \draw[very thin] (LB) -- (RB);
  \draw[very thin] (f) .. controls +(0, -0.4) and +(0, -0.4) .. (e);
  \draw[red, postaction={draw, decorate}] (al) .. controls +(0, -0.6)  and +(0, -0.6) .. (br);
  \draw[red, postaction={draw, decorate}] (ar) .. controls +(0, -1)  and +(0, -1) .. (bl);
\end{scope}

\end{scope}
